DarkSHINE Baseline Design Report: Physics Prospects and Detector Technologies

DarkSHINE is a newly proposed fixed-target experiment initiative to search for the invisible decay of Dark Photon via missing energy/momentum signatures, based on the high repetition rate electron beam to be deployed/delivered by the Shanghai High repetition rate XFEL and Extreme light facility (SHINE). This report elaborates the baseline design of DarkSHINE experiment by introducing the physics goals, experimental setups, details of each sub-detector system technical designs, signal and backgground modelings, expected search sensitivities and future prospects, which mark an important step towards the further prototyping and technical demonstrations.

==> Detectors/ECAL/Future.tex <==
\subsection{Future Optimization}
\label{sec:ECALFuture}

\subsubsection{Staggered geometry}
\label{sec:ECALSiPMGain}

As the central detector of DarkSHINE, the ECAL must be capable of accurately measuring the energy of recoil electrons and bremsstrahlung photons, while minimizing the leakage of electromagnetic showers into the HCAL. Such leakage could result in the dark photon signal being vetoed by the HCAL and also cause electrons from the inclusive background to deposit less energy in the ECAL, leading to misidentification as signal. To maximize the detector's sensitivity to dark photons while minimizing background, we investigated the causes of energy leakage into HCAL. The primary reason is that particles can pass through gaps between the crystals, penetrating the ECAL and reaching the HCAL. Although this occurrence is rare, it directly interferes with our ability to distinguish the dark photon signal. We can reduce or even eliminate such occurrences by optimizing the geometric arrangement of the ECAL. 

\begin{figure}[h]
\centering
    \subfigure[]{
    \includegraphics[width=0.25\textwidth]{Detectors/Figures/ECAL/ECALStaggered.png}}
    \subfigure[]{
    \includegraphics[width=0.33\textwidth]{Detectors/Figures/ECAL/ECALEnergy_8GeV_com_v1.0.pdf}}
    \subfigure[]{
    \includegraphics[width=0.33\textwidth]{Detectors/Figures/ECAL/ECALSignalEfficiency_com.pdf}}
\caption{\label{fig:ECALStaggered}~(a) ECAL with staggered structure, where the placement of crystals in successive layers is shifted by half the transverse dimension of a crystal. (b) Deposited energy of 8 GeV electrons in ECAL with uniform layout and staggered layout. (c) Signal efficiencies in of ECAL with  uniform layout and staggered layout.}
\end{figure}

Figure~\ref{fig:ECALStaggered} (a) shows a staggered layout as a potential geometric configuration. In each layer, the crystals are still positioned in a uniform 21$\times$21 square pattern, which is same as the current design. However, to prevent particles from traversing the gaps, the placement of crystals in successive layers is shifted by half the transverse dimension of a crystal. This staggered structure can effectively reduce energy leakage in the ECAL. Figures~\ref{fig:ECALStaggered} (b) and (c) respectively show a comparison of the energy distribution of the inclusive background and the signal efficiency between the current uniform layout of the ECAL and the staggered layout of the ECAL. 

Compared to the uniform ECAL, the staggered ECAL allows fewer background events to enter the signal region of ECAL, where the ECAL energy is less than 2.5 GeV. In Figure~\ref{fig:ECALStaggered} (b), the ratio of background events entering the ECAL signal region to the total number of events is 1 in 100,000 for the staggered ECAL, with the only event being a hard muon event. In contrast, the uniform ECAL shows a ratio of 381 in 100,000, which is several orders of magnitude higher than the staggered ECAL. Additionally, Figure~\ref{fig:ECALStaggered} (c) shows that the staggered ECAL has a higher signal efficiency.

In the future, to achieve higher sensitivity to dark photons in DarkSHINE experiment, we will conduct further studies on the performance of the ECAL and continue to optimize its geometric structure.

==> Detectors/ECAL/Introduction.tex <==
\subsection{Introduction}
\label{sec:ECALIntroduction}

\subsubsection{Characteristics of signal and background in ECAL}
\label{sec:ECALSignal}

Signal and background processes exhibit distinct characteristics within ECAL. Typically, incident electrons pass through the target with negligible energy loss, deposit most energy in the ECAL, with minimal signals detected by the HCAL. Since in most cases, the particles hitting the ECAL are recoil electrons and bremsstrahlung photons, which could generate electromagnetic showers in the ECAL, leading to significant energy deposition. However, hard processes involving production of high energy muon pairs or hadrons tend to deposit only a small fraction of energy in the ECAL, but they can be effectively rejected using the tracker and HCAL. In Figure~\ref{fig:ECALEnergyTheta} (a), the gray histogram shows the absorbed energy by ECAL for inclusive backgrounds. 

When a dark photon is produced during the electron-on-target process, most of the incident energy transfers to it, and the recoiled electron deposits its remaining energy in the ECAL. The dark photon decays into dark matter, leaving no signal in the tracker or calorimeter, causing significant energy loss in the ECAL. In Figure~\ref{fig:ECALEnergyTheta} (a), more than 75\% of the events have energy deposits in the ECAL that are less than 4 GeV for 1 MeV dark photon signals. While for the inclusive background, only a few events with hard muons or hadrons generated will have deposited energy less than 4 GeV in the ECAL. Therefore, the total energy in the ECAL is an effective selection criterion for the dark photon signal. Otherwise, as the dark photon mass increases, it carries more energy from the electrons, leading to larger recoil angle (Figure~\ref{fig:ECALEnergyTheta} (b)). So the volume of the ECAL should be large enough to maintain high signal acceptance efficiency.

\begin{figure}[h]
\centering  
\subfigure[]{
%\includegraphics[width=0.35\textwidth]
\includegraphics[width=0.45\textwidth]
{Detectors/Figures/ECAL/ECALSignalEnergy_SignalInc_v1.0_py.pdf}}
\subfigure[]{
%\includegraphics[width=0.35\textwidth]
\includegraphics[width=0.45\textwidth]
{Detectors/Figures/ECAL/RecoilTheta_v1.0_py.pdf}}
\caption{\label{fig:ECALEnergyTheta}~
Distributions of ECAL energy (a) and recoil angle of electrons (b) for dark photon signals and inclusive backgrounds.}
\end{figure}

% The ECAL is primarily used to filter out processes with minimal energy loss without production of hard muons or hadrons. 

\subsubsection{Conceptual design}
\label{sec:ECALConceptual}

The ECAL in the DarkSHINE experiment is designed for precise measurement of the energy of recoil electrons and bremsstrahlung photons. As a fixed-target experiment, the DarkSHINE detector will operate under high-frequency electron beams, requiring the detector to have a fast response time and strong radiation resistance. On the other hand, the ECAL should be large enough to absorb all electromagnetic (EM) shower components, reducing EM shower leakage outside of ECAL which could mimick the missing energy signature of dark photon signal.

The ECAL in DarkSHINE experiment is designed to be a homogeneous LYSO crystal calorimeter. LYSO\cite{1239590} is an excellent choice for the crystal material, not only because of its high light yield, which is critical for electromagnetic resolution, but also due to its rapid scintillation decay time (40 ns) and good radiation resistance for handling the extremely high event rate and radiation dose.

\begin{figure}[h]
\centering
%\includegraphics[width=0.4\linewidth]
\includegraphics[width=0.6\textwidth]
{Detectors/Figures/ECAL/ECALStructure_v1.0.png}
    \caption{\label{fig:ECALStructure}~Structure of DarkSHINE ECAL, which consists of an array of LYSO crystal units, each coupled with one SiPM for readout at the end.}
\end{figure}

The structure of ECAL is illustrated in Figure~\ref{fig:ECALStructure}. The transverse dimension of the ECAL is about 50$\times$50 cm$^2$, with a dimension along the beam direction around 44 cm, approximately equivalent to 39 radiation lengths. The substantial volume ensures excellent energy containment in the ECAL, preventing EM showers from leaking into the HCAL. The volume of ECAL is determined by balancing the signal efficiency and crystal cost. The ECAL is fully segmented to gather comprehensive information, enhancing its capability to discriminate dark photons. It is composed of 20$\times$20$\times$11 LYSO crystals, with each crystal measuring 2.5$\times$2.5$\times$4.0 cm$^3$ covered by aluminum film and read out by SiPMs\cite{KLANNER201936, SIMON201985}. The individual crystal size of 2.5$\times$2.5$\times$4.0 cm$^3$ is determined by the maximum density that our electronics can handle~\cite{guo2024}.

==> Detectors/ECAL/Performance.tex <==
\subsection{ECAL expected performance}
\label{sec:ECALPerformance}

\subsubsection{Energy distribution}
\label{sec:ECALEnergyDistribution}
%%ECAL能量分布、单晶体能量分布、shower profile

As a fixed target experiment, incident particles without significant energy loss primarily hit the central area of the ECAL, resulting in substantial energy deposition in the central region's crystals in the first few layers. Additionally, the energy absorbed by crystals in different regions varies greatly, with those closer to the edges typically experiencing minimal energy deposition. To determine the energy dynamic range of the ECALs, the energy deposition in crystals from different regions was investigated.

With the ECAL geometry described in \ref{sec:ECALIntroduction}, the energy deposition in crystals for dark photon signals and background processes is shown in Figure~\ref{fig:ECALEDis} (a). Inclusive background processes typically lead to larger energy deposits in the crystals, reaching up to 4 GeV. While the energy deposition from dark photon signals is lower, with smaller mass dark photons depositing more energy. 

\begin{figure}[htbp]
\centering
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]
    {Detectors/Figures/ECAL/ECell_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]
    {Detectors/Figures/ECAL/Longitudinal_Ratio_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]
    {Detectors/Figures/ECAL/Transverse_Ratio_py.pdf}}
\caption{\label{fig:ECALEDis}~(a) The energy deposited in individual crystals in the ECAL. For inclusive background processes, the energy absorbed by a single crystal can reach up to 4 GeV, while for dark photon signal, it can reach up to 3.5 GeV. (b) Longitudinal shower profiles. (c) Transverse shower profiles.}
\end{figure}

As shown in Figure~\ref{fig:ECALEnergyTheta} (b), with the increase in dark photon mass, the recoil electrons exhibit a progressively wider angular distribution, meaning that EM showers in the ECAL are more likely to occur near the edges of the ECAL. Figure~\ref{fig:ECALEDis} (b) and (c) present the shower profiles within the ECAL for different processes. For the longitudinal shower profile (Figure~\ref{fig:ECALEDis} (b)), the maximum energy deposition for the inclusive background occurs in the second to third layer, while for the dark photon signal, it occurs in a smaller depth. As the dark photon mass increases, the position of the layer with the maximum energy deposition shifts forward, due to the decreasing energy of the recoil electron as the dark photon mass increases. For the transverse shower profile (Figure~\ref{fig:ECALEDis} (c)), the profile width for the dark photon process is larger than that of the inclusive background, showing more energy deposition in crystals located away from the detector's central axis, as it has a larger recoil angle. Moreover, the profile width increases with the increasing mass of the dark photon.


\subsubsection{Energy resolution}
\label{sec:ECALEnergyResolution}
  
The performance of the ECAL can be evaluated by applying digitization to each channel. Figure~\ref{fig:ECALResolution} show the energy resolution and energy containment of the ECAL to 1-8 GeV single electrons. In simulation, the target and other detectors are not included.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.25\linewidth]{Detectors/Figures/ECAL/DIgitization_ECAL_v3.pdf}
%     \caption{\label{fig:ECALResolution}~Energy resolution and energy containment of the ECAL for 1–8 GeV incident electrons, without the target and other detectors. The x-axis represents the energy of the incident electrons. The top figure displays the ECAL's energy resolution, with the fitted stochastic term achieving better than 2\%. The bottom figure shows the energy containment, defined as the ratio of the energy deposited in the ECAL to the incident energy.
%     }
% \end{figure}

\begin{figure}[htbp]
\centering
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECALEnergy_8GeV_v1.0_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_Resolutions_v1.0_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_Linearity_v1.0_py.pdf}}
\caption{\label{fig:ECALResolution}~(a) ECAL energy distributions of 8 GeV electrons for the truth and digitization information. Energy resolution (b) and energy linearity (c) of the ECAL for 1–8 GeV incident electrons, without the target and other detectors. The x-axis represents the energy of the incident electrons.}
\end{figure}

The deposited energy of 8 GeV electrons in ECAL are shown in Figure~\ref{fig:ECALResolution} (a). After digitization, due to the effect of smearing, the energy distribution within the ECAL broadens. This indicates that the detector's resolution has been applied to the original truth energy deposition, resulting in the energy resolution after digitization being worse than that before digitization. The energy resolutions for electrons with different energies are plotted in Figure~\ref{fig:ECALResolution} (b). The statistical term of ECAL's digitized energy resolution can be better than 2\%, thanks to the very high intrinsic light yield of LYSO crystal. The high energy resolution will allow for more precise measurement of recoil electron energy and enhance the reliability in distinguishing between signal and background. Figure~\ref{fig:ECALResolution} (c) shows the energy linearity of ECAL. The overall linearity of the ECAL response is great, except that the measured energy is slightly lower than the incident energy, which is due to the absorption by passive materials in the ECAL and some invisible energy components.

\subsubsection{Signal efficiency}
\label{sec:ECALSignalEfficiency}

Since the total energy in the ECAL is a key criterion on distinguishing the dark photon signal from the background, the signal region is defined as having a total energy in the ECAL of less than 2.5 GeV. This signal region is designed to achieve low background within $3 \times 10^{14}$ electrons-on-target events. It is derived from the combined analysis of all sub-detectors, using thresholds for the ECAL and other sub-detectors, and applying extrapolation methods to exclude all backgrounds\cite{Chen:2022liu}.

\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{Detectors/Figures/ECAL/ECALSignalEfficiency_v1.0_py.pdf}
    \caption{\label{fig:ECALSignalEfficiency}~Signal efficiencies of ECAL for dark photon with various masses. ECAL signal efficiency is defined as the ratio of the number of events with ECAL energy less than 2.5 GeV to the total number of simulated events.}
\end{figure}

The signal efficiency of the ECAL is defined as the ratio of the number of events entering the ECAL signal region to the total number of simulated events. Signal efficiencies for various dark photon masses is shown in Figure~\ref{fig:ECALSignalEfficiency}. As the mass of the dark photon increases, the signal efficiency of the ECAL gradually improves, since higher-mass dark photons tend to carry away more energy, resulting in less energy deposition within the ECAL. Although this also leads to a larger recoil angle, our ECAL is large enough to accept them.

\subsubsection{Reconstructed variables}
\label{sec:ECALReconstructedVariables}

As mentioned earlier, the total ECAL energy can be used to distinguish between inclusive background and dark photon signals. Furthermore, by reconstructing ECAL cell information, variables characterized shower features within the ECAL can be obtained, which can help separate dark photon signals from rare backgrounds. For example, the hadronic showers generated by Photon-Nuclear or Electron-Nuclear processes exhibit different features from electromagnetic showers in the ECAL. Hadrons typically have a larger number of hits and initiate showers deeper within the ECAL than EM showers. Figure~\ref{fig:ECAL_shower_variables} illustrates the distributions of several reconstructed variables for rare backgrounds and dark photon processes, with definitions provided in Table~\ref{tab:ECAL_shower_variable}. It is evident that dark photon processes and these rare processes display distinct distribution patterns, suggesting that reconstruction information can be used to enhance background rejection. It should be noted that the effectiveness of reconstruction is closely linked to the ECAL granularity, and further studies on the ECAL granularity and reconstruction will be conducted in the future.

% The shower variables reconstructed from the high granularity information of ECAL energy deposition in each cell, encoded rich knowledge of the physics process. The definition of the shower variables are defined in Section~\ref{sec:ECALReconstruction} and the separation power are shown in Figure~\ref{fig:ECAL_shower_variables}. The multi-variate method based on Gradient Boosted Decision Tree~\cite{BDT} is developed to efficiently extract the information from all the sensitive shower variables and the distribution of combined score and background suppression power is shown in Figure~\ref{fig:ECALBDTRejection}, highlighted the enhanced separation power of the typical background v.s. signal (10MeV) and fully exploit the granularity of ECAL design. At 99\% signal efficiency, the background is suppressed with a factor up to 748.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Nhit.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Showerden.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Showerrad.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Showerlay.png} \\
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Xwid.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Ywid.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Max3x3x3.png}
%     \includegraphics[width=0.2\linewidth]{Detectors/Figures/ECAL/Max7x7x7.png}
%     \caption{\label{fig:ECAL_shower_variables} Distribution of Shower Variables: N hit, shower density, shower radius, shower layer, X-width, Y-width, Max3x3x3, Max7x7x7}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.95\linewidth]{Detectors/Figures/ECAL/rec_distribution.pdf}
%     \caption{\label{fig:ECAL_shower_variables}~Distributions of several reconstructed variables.}
% \end{figure}

\begin{figure}[htbp]
\centering
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_Edep_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_nhits_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_Emean_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_hit_layer_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_shower_density_py.pdf}}
    \subfigure[]{
    \includegraphics[width=0.32\textwidth]{Detectors/Figures/ECAL/ECAL_shower_layer_py.pdf}}
\caption{\label{fig:ECAL_shower_variables}~Distributions of several reconstructed variables.}
\end{figure}

% \subsubsection{Multiple variables analysis}
% \label{sec:ECALMVA}
% BDT for signal and background separation. Figure~\ref{fig:ECALBDTCorrelation}~\ref{fig:ECALBDTRejection}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{Detectors/Figures/ECAL/BDT_Correlation_bkg.pdf}
%     \caption{\label{fig:ECALBDTCorrelation} BDT Correlation.}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{Detectors/Figures/ECAL/BDT_Rejection.pdf}
%     \caption{\label{fig:ECALBDTRejection} BDT Rejection.}
% \end{figure}



==> Detectors/Target/Background.tex <==
\subsection{Background Processes from Electron-On-Target}
\label{sec:bkgflow}

In most cases, the electrons in the beam pass through the target without any interaction. These events, which are relatively easy to distinguish from signal process leave distinct tracks in the recoil tracker and result in a plentiful energy deposit. However, due to the presence of sufficient material within the target, electrons have potential to occur other processes as they pass through. 

A small fraction of electrons generate additional photons via hard bremsstrahlung process. These bremsstrahlung photons may either contribute to an electromagnetic shower within the ECAL or end up in conversion into hadrons or lepton pairs, which can occur at both target or ECAL. The latter cases are more difficult to distinguish from signal process in ECAL and tracker. These backgrounds are illustrated in Fig~\ref{fig:flowbackground}.

Besides photon conversion, these bremsstrahlung photons can also undergo interactions with materials in the target and ECAL, leading to photon-nuclear reactions that result in hadron production. 

While some of these backgrounds can be easily rejected using single variables, the remaining ones require a combination of information from three sub-detectors for rejection. Although the branch ratios of these processes are relatively small, they cannot be ignored due to the high repetition rate of electron-on-target events, and effectively suppressing these events is crucial for achieving low background expectations.

Moreover, there exist irreducible physics backgrounds that encompass neutrino processes. There are two leading irreducible reactions. The first process is Moller scattering, followed by the charged-current quasi-elastic (CCQE) reaction $e^{-}p \rightarrow \nu_{e}n$. Subsequently, neutrino pair production occurs in the process $e^{-}N \rightarrow e^{-}N\nu\bar{\nu}$, where these neutrinos can acquire a significant fraction of the incident electron's energy. Nevertheless, due to their negligible impact and an approximate rate four orders of magnitude lower than that of 3$\times$10$^{14}$ Electron-On-Target~(EOT), these backgrounds will not be addressed. 

==> Detectors/Tracking/Electronics.tex <==
\subsection{Tracking Electronics}

The DarkSHINE experiment, operating at a high event rate of 1 MHz, demands a robust and high-speed readout system for its tracking detectors. To handle such a high repetition data stream, the tracking electronics must be capable of rapidly processing and transmitting data without introducing significant dead time, which could otherwise compromise the experiment's sensitivity to rare signal events such as dark photon decays. The tracking system is built with the AC-LGAD-based silicon strip detectors, which provide high spatial and temporal resolution. These detectors generate analog signals in response to the passage of charged particles, and the readout electronics must efficiently digitize these signals while maintaining the fine spatial resolution of 10 micrometers and the precise timing requirements.

For its phase-II upgrade, the ATLAS experiment has developed radiation hard high-speed readout ASICs and Front-End electronics. The detector will be operating at instantaneous luminosity up to $7.5\times 10^{34} cm^{-2}s^{-1}$ and 25 ns of bunch-crossing interval (corresponding to 40 MHz). The High Granularity Timing Detector (HGTD) has employed AC-LAGD technology~\cite{Missio:2024hqu}. The 225 channels front-end ATLTIROC (ATLAS LGAD Timing Integrated Read Out Chips) ASICs ~\cite{Agapopoulou:2023jsd} has been tested successfully. The team has been involved in this project. Thus, similar technology can be used for the DarkSHINE tracking electronics, to meet the stringent demands of high repetition rate operation, providing rapid data processing, efficient signal amplification, and reliable synchronization, all while ensuring that the experiment maintains its sensitivity to dark photon searches.



==> Detectors/Tracking/Module.tex <==
\subsection{Tagging Module}

Module test performances


==> Detectors/Tracking/Performance.tex <==
\subsection{Tracking detector module and expected performances}

Based on the tracking detector requirements outlined in the previous sections, a silicon strip detector module has been developed using AC-LGAD technology. The I-V and C-V characteristics of the silicon strip sensor have been thoroughly studied to assess its performance. Its spatial and temporal resolutions have been measured using a laser system, ensuring that the detector meets the necessary precision for the experiment.

To meet the spatial-resolution requirement and study the performance of the detector, three types of strip sensors with pitch (strip) sizes of 100 (50) $\mu m$, 60 (40) $\mu m$, and 45 (30) $\mu m$ were designed for the DarkSHINE experiment, where the strip size refers to the width of the metal strips and electrodes. Two batches of wafers of AC$-$LGAD strip$-$sensor prototypes were produced by the Institute of Microelectronics of the Chinese Academy of Sciences, based on the AC$-$LGAD technology designed by the Institute of High Energy Physics of the Chinese Academy of Sciences (IHEP). They are referred to as the wafer$-$11 and wafer$-$12 sensors hereafter. The n+ doses of these two wafers are 0.01 P and 10 P, respectively, where P is the unit of phosphorus dose defined for the AC-LGADs. Figure~\ref{fig:TrackerIVCV} shows current$-$voltage (left) and capacitance$-$voltage curves of the prototype strip sensors measured at room temperature.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\linewidth]{Detectors/Figures/Tracker/TrackerPerformanceIV.pdf}
\includegraphics[width=0.45\linewidth]{Detectors/Figures/Tracker/TrackerPerformanceCV.pdf}
\caption{\label{fig:TrackerIVCV}~Left: I-V. Right: C-V}
\end{figure}

The position reconstruction performance of the silicon strip detector is key to the DarkSHINE experiment. These aspects are investigated using a laser system with precisely defined positions. Figure~\ref{fig:TrackerPositionSetup} left plot shows the equipment and wiring setup. The right plot shows the silicon strips detector module, i.e a sensor bonded to a 4-channel readout PCB board using aluminium wire.

\begin{figure}[h]
\centering
\includegraphics[width=0.42\linewidth]{Detectors/Figures/Tracker/TrackerLaserTestSetup.png}
\includegraphics[width=0.42\linewidth]{Detectors/Figures/Tracker/TrackerLaserTestModule.jpg}
\caption{\label{fig:TrackerPositionSetup}~Equipment and wiring setup for the position test. Left: schematic diagram of the laser TCT platform. Right: picture of sensor bonded to a 4-channel readout PCB board
using aluminium wire.}
\end{figure}

A detailed analysis of the position resolution measurements and their standard deviations is provided in reference ~\cite{Liu:2023iip}. As illustrated in Figure~\ref{fig:TrackerPositionResult}, the spatial resolution ranged from 6.5 $\mu m$ to 8.2 $\mu m$ for the wafer-11 sensor, and from 8.8 $\mu m$ to 12.3 $\mu m$ for the wafer-12 sensor. The typical sensor response time was approximately 1 $ns$. Wafer-11 exhibited better spatial resolution due to its lower $n^{+}$ dose. Nevertheless, both wafer-11 and wafer-12 sensors meet the spatial resolution requirements for the DarkSHINE experiment.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\linewidth]{Detectors/Figures/Tracker/TrackerStripsBonding.jpeg}
\includegraphics[width=0.45\linewidth]{Detectors/Figures/Tracker/TrackerPositionRes.pdf}
\caption{\label{fig:TrackerPositionResult}~Left: Schematic diagram of sensor strips. Two lines along the x coordinate indicate the paths along which the laser spot moves. C1 to C4 represent the location on the four strips wire bonded for signal readout. Right: Distribution of spatial resolution with respect to x coordinates. The blue and red marks represent the reconstructed position for wafer-11 and wafer-12 sensor, respectively. The circle represents measurement from line-1, while triangle represents measurement from line-2.}
\end{figure}




==> title.tex <==
\makeatletter
\newcommand{\maketitleLARGER}{%
\begin{titlepage}
\let\footnotesize\small
\let\footnoterule\relax
\let \footnote \thanks

\null
\thispagestyle{empty}
\pagestyle{plain}
\pagenumbering{arabic}
\vskip -1.5cm
\vskip 1.0cm

\begin{center}
\vskip 2.cm
\vskip 2cm {\bf \fontsize{50pt} \baselineskip \textbf{DarkSHINE} \par}
\vskip 0.1em
\vskip 1cm {\bf \fontsize{35pt} \baselineskip  \textit{Baseline Design Report} \par}
\vskip 0.1em
\vskip 1mm {\bf \huge \textsf{Physics Prospects and Detector Technologies} \par}
\vskip 0.3em
\vskip 1mm { \Huge \baselineskip 1.5cm \textsf{Version 1} \par}
\vskip 10cm

{
% \large
\small 
\lineskip .70em
\baselineskip 1cm
\newpage
% \vspace*{3cm}
\begin{tabular}[t]{p{\textwidth}} % {c}
{ \centering \@author \par }
\end{tabular}
}
\vskip 0.6em
\vskip 1mm 
{\bf \Large \textsf{\today}}

\end{center}\par    

\end{titlepage}
\setcounter{footnote}{0}
\setcounter{page}{1}
}
\makeatother
